Spectral Formation in Accreting X-Ray Pulsars: Bimodal Variation of the Cyclotron Energy with Luminosity

Accretion-powered X-ray pulsars exhibit significant variability of the Cyclotron Resonance Scattering Feature (CRSF) centroid energy on pulse-to-pulse timescales, and also on much longer timescales. Two types of spectral variability are observed. For sources in group 1, the CRSF energy is negatively correlated with the variable source luminosity, and for sources in group 2, the opposite behavior is observed. The physical basis for this bimodal behavior is currently not understood. We explore the hypothesis that the accretion dynamics in the group 1 sources is dominated by radiation pressure near the stellar surface, and that Coulomb interactions decelerate the gas to rest in the group 2 sources. We derive a new expression for the critical luminosity such that radiation pressure decelerates the matter to rest in the supercritical sources. The formula for the critical luminosity is evaluated for 5 sources, using the maximum value of the CRSF centroid energy to estimate the surface magnetic field strength. The results confirm that the group 1 sources are supercritical and the group 2 sources are subcritical, although the situation is less clear for those highly variable sources that cross over the critical line. We also explain the variation of the CRSF energy with luminosity as a consequence of the variation of the characteristic emission height. The sign of the height variation is opposite in the supercritical and subcritical cases, hence creating the observed bimodal behavior.

==> XXXXaasm.tex <==
%
%  These Macros are taken from the AAS TeX macro package version 4.0.
%  Include this file in your LaTeX source only if you are not using
%  the AAS TeX macro package and need to resolve the macro definitions
%  in the BibTeX entries returned by the ADS abstract service.
%
%  For more information on the AASTeX macro package, please see the URL
%	http://www.aas.org/publications/aastex.html
%  For more information about ADS abstract server, please see the URL
%	http://adswww.harvard.edu/ads_abstracts.html
%

% Abbreviations for journals.  The object here is to provide authors
% with convenient shorthands for the most "popular" (often-cited)
% journals; the author can use these markup tags without being concerned
% about the exact form of the journal abbreviation, or its formatting.
% It is up to the keeper of the macros to make sure the macros expand
% to the proper text.  If macro package writers agree to all use the
% same TeX command name, authors only have to remember one thing, and
% the style file will take care of editorial preferences.  This also
% applies when a single journal decides to revamp its abbreviating
% scheme, as happened with the ApJ (Abt 1991).

\def\jnl@style{\it}
%commente par Seb
\def\aaref@jnl#1{{\jnl@style#1}}
%ref remplace par aaref pour eviter conflit...

\def\aaref@jnl#1{{\jnl@style#1}}

\def\aj{\aaref@jnl{AJ}}                   % Astronomical Journal
\def\araa{\aaref@jnl{ARA\&A}}             % Annual Review of Astron and Astrophys
\def\apj{\aaref@jnl{ApJ}}                 % Astrophysical Journal
\def\apjl{\aaref@jnl{ApJ}}                % Astrophysical Journal, Letters
\def\apjs{\aaref@jnl{ApJS}}               % Astrophysical Journal, Supplement
\def\ao{\aaref@jnl{Appl.~Opt.}}           % Applied Optics
\def\apss{\aaref@jnl{Ap\&SS}}             % Astrophysics and Space Science
\def\aap{\aaref@jnl{A\&A}}                % Astronomy and Astrophysics
\def\aapr{\aaref@jnl{A\&A~Rev.}}          % Astronomy and Astrophysics Reviews
\def\aaps{\aaref@jnl{A\&AS}}              % Astronomy and Astrophysics, Supplement
\def\azh{\aaref@jnl{AZh}}                 % Astronomicheskii Zhurnal
\def\baas{\aaref@jnl{BAAS}}               % Bulletin of the AAS
\def\jrasc{\aaref@jnl{JRASC}}             % Journal of the RAS of Canada
\def\memras{\aaref@jnl{MmRAS}}            % Memoirs of the RAS
\def\mnras{\aaref@jnl{MNRAS}}             % Monthly Notices of the RAS
\def\pra{\aaref@jnl{Phys.~Rev.~A}}        % Physical Review A: General Physics
\def\prb{\aaref@jnl{Phys.~Rev.~B}}        % Physical Review B: Solid State
\def\prc{\aaref@jnl{Phys.~Rev.~C}}        % Physical Review C
\def\prd{\aaref@jnl{Phys.~Rev.~D}}        % Physical Review D
\def\pre{\aaref@jnl{Phys.~Rev.~E}}        % Physical Review E
\def\prl{\aaref@jnl{Phys.~Rev.~Lett.}}    % Physical Review Letters
\def\pasp{\aaref@jnl{PASP}}               % Publications of the ASP
\def\pasj{\aaref@jnl{PASJ}}               % Publications of the ASJ
\def\qjras{\aaref@jnl{QJRAS}}             % Quarterly Journal of the RAS
\def\skytel{\aaref@jnl{S\&T}}             % Sky and Telescope
\def\solphys{\aaref@jnl{Sol.~Phys.}}      % Solar Physics
\def\sovast{\aaref@jnl{Soviet~Ast.}}      % Soviet Astronomy
\def\ssr{\aaref@jnl{Space~Sci.~Rev.}}     % Space Science Reviews
\def\zap{\aaref@jnl{ZAp}}                 % Zeitschrift fuer Astrophysik
\def\nat{\aaref@jnl{Nature}}              % Nature
\def\iaucirc{\aaref@jnl{IAU~Circ.}}       % IAU Cirulars
\def\aplett{\aaref@jnl{Astrophys.~Lett.}} % Astrophysics Letters
\def\apspr{\aaref@jnl{Astrophys.~Space~Phys.~Res.}}
                % Astrophysics Space Physics Research
\def\bain{\aaref@jnl{Bull.~Astron.~Inst.~Netherlands}} 
                % Bulletin Astronomical Institute of the Netherlands
\def\fcp{\aaref@jnl{Fund.~Cosmic~Phys.}}  % Fundamental Cosmic Physics
\def\gca{\aaref@jnl{Geochim.~Cosmochim.~Acta}}   % Geochimica Cosmochimica Acta
\def\grl{\aaref@jnl{Geophys.~Res.~Lett.}} % Geophysics Research Letters
\def\jcp{\aaref@jnl{J.~Chem.~Phys.}}      % Journal of Chemical Physics
\def\jgr{\aaref@jnl{J.~Geophys.~Res.}}    % Journal of Geophysics Research
\def\jqsrt{\aaref@jnl{J.~Quant.~Spec.~Radiat.~Transf.}}
                % Journal of Quantitiative Spectroscopy and Radiative Transfer
\def\memsai{\aaref@jnl{Mem.~Soc.~Astron.~Italiana}}
                % Mem. Societa Astronomica Italiana
\def\nphysa{\aaref@jnl{Nucl.~Phys.~A}}   % Nuclear Physics A
\def\physrep{\aaref@jnl{Phys.~Rep.}}   % Physics Reports
\def\physscr{\aaref@jnl{Phys.~Scr}}   % Physica Scripta
\def\planss{\aaref@jnl{Planet.~Space~Sci.}}   % Planetary Space Science
\def\procspie{\aaref@jnl{Proc.~SPIE}}   % Proceedings of the SPIE

\let\astap=\aap
\let\apjlett=\apjl
\let\apjsupp=\apjs
\let\applopt=\ao



==> XXXXmyma.tex <==
\usepackage{xspace}

\newcommand{\ecs}{\ensuremath{ \mathrm{erg~cm^{-3}~s^{-1}}}}
\newcommand{\ergmpc}{\ensuremath{ \mathrm{erg~s^{-1}~Mpc^{-3}}}}
\newcommand{\msol}{\ensuremath{\mathrm{M}_{\odot}}}
\newcommand{\msoly}{\ensuremath{ \mathrm{M}_{\odot} / \mathrm{yr}^{-1} }}
\newcommand{\lusol}{\ensuremath{\mathrm{L}_{\odot}}}
\newcommand{\eccs}{\ensuremath{ \mathrm{erg\,cm^{-2}\,s^{-1}}}}
\newcommand{\ergs}{\ensuremath{ \mathrm{erg\,s}^{-1} }}
\newcommand{\nh}{\ensuremath{ \mathrm{N _H}}}
\newcommand{\PASP}[1]{{\em Publ. Astron. Soc. of Pac.,\ }{\bf#1}}
\newcommand{\NAT}[1]{{\em Nature,\ }{\bf#1}}
\newcommand{\dd}[2]{\frac{{\rm d}#1}{{\rm d}#2}}
\newcommand{\ddd}[3]{\frac{{\rm d}#1}{{\rm d}#2\,{\rm d}#3}}
\newcommand{\pdd}[2]{\frac{\partial #1}{\partial#2}}
\newcommand{\kms}{\ensuremath{ \mathrm{km~s}^{-1}}}
\newcommand{\fres}{\frenchspacing}
\newcommand{\et}{{\sl et al.\,}}
\newcommand{\micr}{\,\mu{\rm m}}
\newcommand{\gra}{\raisebox{1ex}{\scriptsize o}}
\newcommand{\lulog}{\log_{10}\frac{\lse}{\lusol}}
\newcommand{\gev}{{\ensuremath{ \mathrm{GeV}}}}
\newcommand{\ev}{{\ensuremath{ \mathrm{eV}}}}
\def\Mpc{\,{\rm Mpc}}
\def\la{\mathrel{\mathpalette\fun <}}
\def\ga{\mathrel{\mathpalette\fun >}}
\def\fun#1#2{\lower3.6pt\vbox{\baselineskip0pt\lineskip.9pt
  \ialign{$\mathsurround=0pt#1\hfil##\hfil$\crcr#2\crcr\sim\crcr}}}
% Use $$\Braket{\phi | {\partial^2}\over {\partial t^2} | \psi}$$
\def\bra#1{\mathinner{\langle{#1}|}}
\def\ket#1{\mathinner{|{#1}\rangle}}
\def\braket#1{\mathinner{\langle{#1}\rangle}}
\def\Bra#1{\left<#1\right|}
\def\Ket#1{\left|#1\right>}
{\catcode`\|=\active
  \gdef\Braket#1{\left<\mathcode`\|"8000\let|\bravert {#1}\right>}}
\def\bravert{\egroup\,\vrule\,\bgroup}
\def \arcmin {\hbox{$^\prime$}}
\def \arcsec {\hbox{$^{\prime\prime}$}}
\def\pc{\,{\rm pc}}
\def\kpc{\,{\rm kpc}}
\def\Mpc{\,{\rm Mpc}}
\def\mpc{\,{\rm Mpc}}

\def\gtrsim{\ensuremath{\; \buildrel > \over \sim \;}}
\def\gsim{\lower.5ex\hbox{\gtsima}}
%\def\ga{\mathrel{\mathpalette\fun >}}

%\newcommand{\instrument}[1]{\textsl{#1}\xspace}

\newcommand{\inte}{\textsl{INTEGRAL}\xspace}
\newcommand{\sax}{\textsl{BeppoSAX}\xspace}
\newcommand{\ssax}{\textsl{SAX}\xspace}
\newcommand{\lecs}{\textsl{LECS}\xspace}
\newcommand{\mecs}{\textsl{MECS}\xspace}
\newcommand{\pds}{\textsl{PDS}\xspace}
\newcommand{\hp}{\textsl{HPGSPC}\xspace}
\newcommand{\rxte}{\textsl{RXTE}\xspace}
\newcommand{\pca}{\textsl{PCA}\xspace}
\newcommand{\hexte}{\textsl{HEXTE}\xspace}
\newcommand{\hextea}{\textsl{HEXTE-A}\xspace}
\newcommand{\hexteb}{\textsl{HEXTE-B}\xspace}
\newcommand{\IBIS}{\textsl{IBIS}\xspace}
\newcommand{\SPI}{\textsl{SPI}\xspace}
\newcommand{\JEMX}{\textsl{JEM-X}\xspace}
\newcommand{\prog}[1]{\texttt{#1}\xspace}
\newcommand{\xspec}{\prog{XSPEC}\xspace}
%\newcommand{\flux}{\gamma \ {\rm cm^{-2} s^{-1}}}
\newfont{\mc}{cmcsc10 scaled\magstep2}
\newfont{\cmc}{cmcsc10 scaled\magstep1}
\newcommand {\etal}{{\it et~al. }}
\newcommand{\flux}{{\rm ph\,cm^{-2}\,s^{-1}}}
\newcommand{\eflux}{{\rm erg\,cm^{-2}\,s^{-1}}}
%\newcommand{\src}{4U~0115+63\xspace}
%\newcommand{\fu}{4U~1907+097\xspace}
\newcommand{\fu}{4U~0115$+$63\xspace}
\newcommand{\her}{Her~X-1\xspace}
\newcommand{\cen}{Cen~X-3\xspace}


%\renewcommand{{\`i}}{\`{\i}}

\newcommand{\slap}[2] {\frac{1}{#2 ^2}\frac{{\mathrm d}}{{\mathrm d} #2}\left( #2^2 \frac{{\mathrm d} #1}{{\mathrm d} #2} \right )}

\newcommand{\bgi}{\begin{itemize}}
\newcommand{\edi}{\end{itemize}}

\newcommand{\be}{\begin{equation}}
\newcommand{\ee}{\end{equation}}

\newcommand{\bea}{\begin{eqnarray}}                  %
\newcommand{\eea}{\end{eqnarray}}                    %

\newcommand{\beaa}{\begin{eqnarray*}}                %
\newcommand{\eeaa}{\end{eqnarray*}}                  %

\newcommand{\bgd}{\begin{description}}
\newcommand{\edd}{\end{description}}

\newcommand{\bgf}{\begin{figure}}
\newcommand{\edf}{\end{figure}}

\newcommand{\bgc}{\begin{center}}
\newcommand{\edc}{\end{center}}

\newcommand{\bgt}{\begin{tabular}}
\newcommand{\edt}{\end{tabular}}

\newcommand{\bge}{\begin{enumerate}}
\newcommand{\ede}{\end{enumerate}}

\newcommand{\fns}{\footnotesize}
\newcommand{\REF}{\par\noindent\hangindent 20pt}
 
\DeclareRobustCommand{\ion}[2]{%
 \relax\ifmmode
 \ifx\testbx\f@series
 {\mathbf{#1\,\mathsc{#2}}}\else
 {\mathrm{#1\,\mathsc{#2}}}\fi
 \else\textup{#1\,{\mdseries\textsc{#2}}}%
 \fi}








